Congestion-aware Routing and Rebalancing of Autonomous Mobility-on-Demand Systems in Mixed Traffic

This paper studies congestion-aware route-planning policies for Autonomous Mobility-on-Demand (AMoD) systems, whereby a fleet of autonomous vehicles provides on-demand mobility under mixed traffic conditions. Specifically, we first devise a network flow model to optimize the AMoD routing and rebalancing strategies in a congestion-aware fashion by accounting for the endogenous impact of AMoD flows on travel time. Second, we capture reactive exogenous traffic consisting of private vehicles selfishly adapting to the AMoD flows in a user-centric fashion by leveraging an iterative approach. Finally, we showcase the effectiveness of our framework with two case-studies considering the transportation sub-networks in Eastern Massachusetts and New York City. Our results suggest that for high levels of demand, pure AMoD travel can be detrimental due to the additional traffic stemming from its rebalancing flows, while the combination of AMoD with walking or micromobility options can significantly improve the overall system performance.

==> sections/02_Intro-Mauro.tex <==
\section{Introduction} \label{sec:intro}

\lettrine{I}{n the past} decade, the combination of smartphone technologies and wireless communications with the concept of sharing economies has resulted in a pervasive diffusion of Mobility-on-Demand (MoD) services.
%\MS{Maybe we could add some background information on congestion problems as in my ECC or RSS papers.}
Deciding vehicle routes and rebalancing policies of a fleet is one of the main operational challenges that these platforms face. Currently, MoD systems use routing services (e.g., Waze and Google Maps) to route their vehicles, and provide drivers with a real-time heat-map of users' demand and dynamically adapt their prices in order to rebalance their fleets.
Given this \emph{user-centric} approach to route vehicles, in which every driver acts selfishly to minimize their own travel time, the network reaches an equilibrium known as the \emph{Wardrop} equilibrium~\cite{wardrop1952road}. Unfortunately, these equilibria are in general suboptimal compared to the system optimum achievable when vehicles are coordinated by a central controller in a \emph{system-centric} fashion.

Recently, the combination of MoD services with Connected and Automated Vehicles (CAVs) has attracted the interest of academia and industry, giving rise to Autonomous Mobility-on-Demand (AMoD) systems. These are fleets of CAVs providing on-demand mobility which are expected to reduce labor costs, the number of accidents, and harmful emissions~\cite{guanetti2018control}.
Additionally, these fleets can be centrally controlled and therefore enable for system-optimal routing strategies to be implemented.

In this context, this paper presents system-optimal routing and rebalancing strategies for AMoD systems in mixed-traffic conditions.
%%
\begin{figure}[t]
	\centering
	\includegraphics[width=1\linewidth]{fig/AMODnet.pdf}
	\caption{AMoD network (supergraph) consisting on two DiGraphs for the road (blue) and the walking (orange) network and the black arrows represent switching arcs. AMoD vehicles are in black and private vehicles in grey.}
	\label{fig:road-walking-graph}
	\vspace{-.45cm}
\end{figure}

\emph{Related Literature:}
The models used to study AMoD systems comprise simulation models~\cite{swaszek2019load, HoerlRuchEtAl2018, LevinKockelmanEtAl2017}, queuing-theoretical models~\cite{ZhangPavone2016,IglesiasRossiEtAl2016}, and network-flow models~\cite{PavoneSmithEtAl2012,RossiZhangEtAl2017,SpieserTreleavenEtAl2014}.


Moreover, threshold approximations have been recently used to study congestion effects \cite{RossiZhangEtAl2017}, sometimes capturing the interaction with public transit~\cite{SalazarRossiEtAl2018,SalazarLanzettiEtAl2019} or the power-grid~\cite{RossiIglesiasEtAl2018,RossiIglesiasEtAl2018b}. 
 In~\cite{SoloveySalazarEtAl2019} to rapidly solve the AMoD routing and rebalancing problem capturing BPR-type congestion models. However, such an approach cannot include other means of transportation such as walking or public transit.
Against this backdrop, a piecewise approximation of the BPR function is introduced in~\cite{SalazarTsaoEtAl2019}, whereby convex relaxations are leveraged to frame the congestion-aware routing problem in intermodal settings as a quadratic program.
Yet, depending on the congestion levels, the latter approach may lack in accuracy. Moreover, both methods assume non-reactive exogenous traffic flows.
%Using the user-centric model, Mehr et al. \cite{mehr2019will} under the assumption of shorter headway for CAVs, argue that selfish routing of CAVs may result in an increase in traffic congestion.
Recently, reactive private traffic was modeled in~\cite{houshmand2019penetration} to show that under a system-centric optimal-routing strategy both CAVs and non-CAVs can achieve better performance in terms of travel time and energy savings. However, such an approach does not capture rebalancing effects nor intermodal routing possibilities.

\emph{Statement of contribution:} This paper bridges the gap between~\cite{SalazarTsaoEtAl2019} and~\cite{houshmand2019penetration}. Specifically, we study how system-optimal routing of AMoD services can affect the system-level performance in mixed-traffic conditions. Similar to \cite{SalazarTsaoEtAl2019} we assume that AMoD customers can use multiple modes of transportation, i.e., autonomous taxi rides and walking. In addition, however, we assume private vehicles to be reactive, meaning they will choose their routes selfishly considering the AMoD flow. To this end, we extend the method presented in~\cite{houshmand2019penetration} to capture the interaction between AMoDs and private vehicles (\emph{mixed traffic}). Moreover, we provide a more accurate approximation of endogenous congestion effects, while still maintaining the convex structure of the AMoD problem.
The proposed model can efficiently compute the congestion-aware routing and the rebalancing policy for a given demand and road network topology.
Finally, with this framework at hand, we analyze the trade-offs between the benefit of socially-routing and the cost of rebalancing. In addition, we provide examples of the advantages of providing mobility services by considering both autonomous taxi-rides and walking options.
\MS{What about micromobility?}
Finally, since our model calculates optimal flows, we include an algorithm to recover the routes from the flow-based solution.  

The rest of the paper is organized as follows: In Section~\ref{sec:problem formulation} we provide  preliminaries of the model and its formulation. In Section~\ref{sec:travel-latency-function-approximation} we develop a convex approximation of the original problem to overcome its non-convex nature. Then, we present experiments using the Eastern Massachusetts and New York City road networks. Finally, in Section~\ref{sec:conclusions} we conclude the paper and point to future research directions.

\MS{Would move this to the next section.} \textbf{Notation:} All vectors are column vectors and denoted by bold lowercase letters. Bold uppercase letters denote matrices.  We use ``prime'' to denote the transpose of a matrix or vector. We denote by $\mathbbm{1_x}$ the indicator function. $\|\cdot\|$ denotes the $\ell_2$ norm. 


==> sections/06_Route-recovery.tex <==
\section{Route recovery strategies}

All of the methodologies used in this paper aim to solve the routing problem by choosing flows $\bx^c$ and $\bx^r$ that minimize some metric. Even if these solutions allow us to asses network deficiencies and to plan infrastructure, it does not gives specific routes which vehicles should follow. 

In this section, we present a simple, parallelizable and powerful algorithm to recover the routes which approximate the AMoD flow solution, as well as an algorithm to retrieval the rebalancing routes. 

\subsection{Routes retrieval for OD pairs}
Let the optimal solution of the routing and rebalancing problem be $(\{\bx^{\bw*}\}_{\bw \in \scrW}, \bx^{r*})$. We denote with $\scrR_\bw$ to be  the set of considered routes of OD pair $\bw$. Then, for each $\bw\in \scrW$, we let $\bp$ be a vector with elements $p_{i}$ denoting the percentage of vehicles routed trough route $i \in \scrR_\bw$. Lastly, we use $\bA$ to denote the route-link incidence matrix of $
\scrR_\bw$. With these definitions, one can find the routes by solving the following convex optimization problem.
\begin{flalign}
    \centering
    & \min\limits_{\bp>0}  \| \bA\bp d_\bw - \bx^{\bw*} \| \label{eq:route-finder}
\end{flalign}
where the product $\bA \bp d_\bw$ is equal to the estimated link flow induced by routing the percentage $p_i$ of vehicles trough route $i$.

The problem of selecting which route to include in $\scrR_\bw$ is an interesting one. To solve this, we take the greedy approach of adding the next shortest route for each OD pair, and solving again problem \eqref{eq:route-finder}. To stop the algorithm, we use a user-defined parameter $\xi$ which serves as a stopping criteria. See Alg. \ref{alg:route-recovery}.
It is worth mentioning that this algorithm can be run in parallel for each OD pair, and for not so congested networks we expect the solution to converge fast. This is because when there is few congestion, the majority of vehicles will be routes trough the shortest paths, which are the first ones to be added into $\scrR_\bw$.

\begin{algorithm}[h]
\SetAlgoLined
\footnotesize
\KwResult{Percentage of vehicles following each path}
 initialization\;
 \While{ $\| \bx - \bx^* \| > \xi$}{
    \text{add the next shortest route to the set } $\scrR_\bw$\;
    \text{solve problem } \eqref{eq:route-finder}\;}
 \caption{Route-recovery for a specific OD pair}
 \label{alg:route-recovery}
\end{algorithm}
Interestingly, when networks are at equilibrium, multiple routes connecting a particular OD pair might have the same travelling time. Hence, in order to break ties, one can use any simple random ordering approach. However, the possibility that all equilibrium routes are used by that OD pair is high. Hence, we recommend adding all the tie routes to the set $\scrR$ to speed up the process.

\subsection{Routes retrieval for rebalancing flow}
The problem of obtaining the routes of the rebalancing flow is harder since we do not have distinction between OD pair flow. Given space constraints of this paper we wont formally address the problem, but rather give a sketch of the main idea. 
We propose finding the set of potential origins $\scrO \subset \scrV_R$ and destinations $\scrD \subset \scrV_R$ by scanning every node in the network and computing its potential
\begin{align}
    \psi(j) = \sum_{i:(i,j)\in\scrA_R} x^r_{ij} -\sum_{k:(j,k)\in\scrA_R} x^r_{jk} \label{eq:route-retrival-od-pairs}
\end{align}
for any node $j$.  
If $\psi(j)=0$ the node is in equilibrium and it is not part of an origin or destination of the rebalancing flow. If $\psi(j)>0$ we say that the node $j$ is a destination and we let $j\in \scrD$. Similarly, if $\psi(j)<0$ we set $j$ as an origin and we let $j\in \scrO$.

For each origin $j\in\scrO$ we create $|\scrD|$ destinations, and we let $\scrR_\bw$ be a route set for each rebalancing OD pair $\bw$. Then, we solve a problem similar as in \eqref{eq:route-finder}, but considering multiple OD pairs in the optimization. 

Notice that this strategy might result on having too many OD pairs given its combinatorial nature. To lower the decision space of this problem, we propose using a threshold-based method to avoid creating OD pairs whose origin and destination are far in travel time. In other words, let $\eta_{\bw}$ be a fixed travel time using the shortest path from origin $w_s\in\scrO$ to destination $w_t\in\scrD$. Then, let the travel time to the closest destination $w_d$ of  origin $w_s$ be $\kappa(w_s) = \min \{\eta_{w_s w_t}\}_{w_t \in \scrD}$ .
The threshold-based method ignores a potential OD pair $\bw$ whose $(\eta_{\bw}/\kappa(w_s))-1>\rho$, where $\rho$ is a fixed threshold. 
Note that in this case, the potential rebalancing OD pair $\bw$ will be added to the set if its shortest route in travel time is less than $\rho \%$ higher than the travel time to the closest OD pair of $w_s$. 
